CNNPruner: Pruning Convolutional Neural Networks with Visual Analytics

Convolutional neural networks (CNNs) have demonstrated extraordinarily good performance in many computer vision tasks. The increasing size of CNN models, however, prevents them from being widely deployed to devices with limited computational resources, e.g., mobile/embedded devices. The emerging topic of model pruning strives to address this problem by removing less important neurons and fine-tuning the pruned networks to minimize the accuracy loss. Nevertheless, existing automated pruning solutions often rely on a numerical threshold of the pruning criteria, lacking the flexibility to optimally balance the trade-off between model size and accuracy. Moreover, the complicated interplay between the stages of neuron pruning and model fine-tuning makes this process opaque, and therefore becomes difficult to optimize. In this paper, we address these challenges through a visual analytics approach, named CNNPruner. It considers the importance of convolutional filters through both instability and sensitivity, and allows users to interactively create pruning plans according to a desired goal on model size or accuracy. Also, CNNPruner integrates state-of-the-art filter visualization techniques to help users understand the roles that different filters played and refine their pruning plans. Through comprehensive case studies on CNNs with real-world sizes, we validate the effectiveness of CNNPruner.

==> README <==
Created by Torsten Moeller (vis@cs.sfu.ca), April 6 2004
modified by Steven Bergner and Torsten Moeller, June 30 2006
modified by James Peltier and Torsten Moeller, March 28, 2007
modified by Bernhard Finkbeiner, July 5, 2010
modified by Tobias Isenberg, January 2016
modified by Filip Sadlo, March 2016
modified by Tobias Isenberg, July 2016

This distribution provides a document class for formatting papers according to the specifications for submission to conferences sponsored by the IEEE Visualization & Graphics Technical Committee (VGTC).

Conferences that use the 'journal' document option:
- IEEE Visualization Conference (VIS, incl. InfoVis, SciVis, VAST)
- IEEE Virtual Reality (VR)
- IEEE International Symposium on Mixed and Augmented Reality (ISMAR)

It contains 13 files/directories:

README          - this file
diamondrule.eps - abstract and body separator
diamondrule.pdf - its PDF version
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default journal mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used as such (using the established LaTeX environments) by calling pdfLaTeX or LaTex. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Uinux-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)


==> text/backup_04-27.tex <==
% The following experiments may be deleted
%(\clr{what this paragraph is describing?}) In addition, we carry out visual pruning optimization at the beginning and middle stages of pruning to improve the accuracy for category `buildings'. However, due to the high over-parameterization of the network in these stages, the effect is not good. When the accuracy of the model begins to decline, visual optimization can effectively improve or maintain the accuracy of the specific category. Therefore, in the later stage of pruning, visual optimization of the pruning plan can ensure the accuracy of the specific category.

% For the picture '22479.jpg' in \autoref{fig:intel_evolution}, we can see that after pruning the category of this picture is from category `sea' to category `mountain'.
% Through the visualization of the feature map in the filter, we find that Filter 5 which contains the most clearest sea features is deleted.
% For the picture '21805.jpg' in \autoref{fig:intel_evolution}, Filter 5 with the clearest glacier features is removed.
% Therefore, we think that deleting the filter which is focused on the false features can enhance other features in the fine-tuning process, that it is likely to make the classification of the image correct (R3.2).
% Another interesting phenomenon is that pruning exposes some bad or confusing pictures. 
%

% We think the deletion of Filter 0 and Filter 5 leads to the loss of learning content of category `buildings' in the network, and it is difficult to relearn in the subsequent fine-tuning process.





%\clr{i rewrote this paragraph. Please add the requirement R*.* to proper locations.}

% The input of \sysname{} is a pre-trained CNN model, the information (\clr{what kind of information?}) of which can be automatically detected and presented through the front-end of \sysname{}.
% Then, {\sysname} detects the model information and displays them on the front-end.
% The \textit{Tree} view (\autoref{fig:teaser}a) tracks the whole pruning process and provides an overview of each intermediate pruned CNN model (R1.1).
% This view allows users to estimate the new \clr{node model attributes(?)} between adjacent models through the interaction with the estimator, and then determine the number of filters to be removed (R2.3).

% It provides feedback on the impact of the metrics and the model structure in real-time to help users estimate the influence of the pruning scheme (R2.1). With its helps, users can better, estimate and adjust the number of filters to be removed. 
% Therefore, users can determine the number of removal with the help of the \textit{Model} view, and then adjust it by evaluating the scheme through the \textit{Statistics} view after pruning (R2.2).


% Under the guidance of the system and the operation of the user, {\sysname} helps the user get the desired pruned model.




% Through the information, the user can understand the classification ability of the model for different categories.

% As shown in \autoref{fig:teaser}-b1, the Confusion Matrix displays the accuracy and confusion of each category (R1.2). 
% The labels on the left of the matrix represent the true labels, and the labels on top represent the predict labels.
% In the matrix, cells on the diagonal represent the count of true-positives.
% the accuracy of each category, and the other block is the confusion value between the true label and predict label.
% The definition of confusion value is the percentage of test datasets that the model recognizes from one category to another.
% The darker the color of the block in the matrix, the larger the value.
% When the user clicks on a block in the matrix, this view switches to a line chart to show the value changes for the current label during the pruning process.
% Through the information, the user can understand the classification ability of the model for different categories.



%Convolutional neural networks (CNNs) have demonstrated extraordinarily good performance in many computer vision tasks recently. The increasing size of CNNs, however, also prevents them from being widely deployed to devices with limited resources, e.g., mobile/embedded devices. The emerging topic of \textit{model pruning} strives to address this problem by removing less important neurons and fine-tuning the pruned networks to minimize the accuracy loss. Nevertheless, existing automated pruning solutions often rely on a numerical threshold of the importance criteria for pruning, lacking the flexibility to optimally balance the trade-off between model size and accuracy. Moreover, the complicated state change of neurons over the pruning and fine-tuning makes this process less transparency, and hard to be improved. 
%In this paper, we address these challenges through a visual analytics attempt, named \sysname{}. It leverages the importance of convolutional filters through both instability and sensitivity, and allows users to interactively create pruning plans according to a desired goal on model size or accuracy. Also, \sysname{} integrates state-of-the-art filter visualization techniques to help users understand the roles that different filters played and refine their pruning plans. Through comprehensive case studies on CNNs with real-world sizes, we validate the effectiveness of \sysname{}.



%Convolutional neural networks have demonstrated excellent performance in many computer vision tasks. However, the rapid increase of parameters in the neural network makes some embedded devices unable to run the model. Model pruning can solve this problem without compromising accuracy. But it hard to understand the state change of neural networks in the process of pruning, and make the user difficult to develop a proper pruning schedule.
%In this paper, we present a visual analytics system to help users understand the process and improve the efficiency of model pruning. We use instability and sensitivity to evaluate each filter in the neural network and allow user interaction to analyze the filters and make pruning schedules. Through the filter visualization, users can understand the pruning more deeply and refine the pruning scheme. The system can help users generate a basic pruning process tree by the automatic pruning. Users can optimize the process tree with information on different attributes in the different models and then get the desired compression model. We validate the effectiveness of our system through multiple test cases.


% Different views focus on different levels of information in the pruning process, and they work together to record the state changes of the model in the whole process in detail.
% \sysname{} uses two metrics to evaluate the filter, and three criteria to evaluate the fine-tuning process.
% The user can make and adjust pruning plans through pre-estimation and post-evaluation.
% Using this progressive pruning method can improve the pruning effect and avoid the influence of abnormal model on pruning.
% In addition, by defining degenerated instances and the improved instances, the workload of analysis can be greatly reduced, which is helpful for the user to conduct in-depth analysis and refine the plan.




==> text/backup_text.tex <==

%Each node of the tree represents a CNN model. The root node of the tree is the pre-trained model, and the others are pruned models. We use a rectangle composed of three rectangles to represent the nodes in the tree, where the number in the left rectangle is the model id, the upper right rectangle represents the accuracy rate and the lower right rectangle represents the compression rate. The connection between nodes in the tree is in black and red. The black line indicates that the fine-tuning process after pruning from the parent node to the child node reaches the convergence condition which is set by the user, and the red line indicates the fine-tuning process achieves the maximum number of epoch without convergence. The leftmost axis in the \textit{Tree} View is represents the number of filters, and this axis only shows the number of filters corresponding to the model in the right tree. There is also an estimator in the \textit{Tree} View to show the estimated accuracy and compression rate under a specified number of filters. The toolbar is in the upper side of the \textit{Tree} View.

% interaction
%Tree view allows users to select nodes in the tree and switch the right information according to the selected model.

%Users need to load a pre-trained CNN model first when using the system, and configure the training set parameter, test set parameter, fine-tuning parameters, auto-pruning parameters, etc. through the configuration box provided by the toolbar. Then the system can generate a basic tree through automatic pruning and users can select a node as the start point and make a pruning plan by using the estimator and model detail information. After the iterative pruning, the user can export the target model and complete the pruning.


In this section we discuss some of the concepts proposed in this paper.

\subsection{Sensitivity and Instability}
In our work, we use the ${Sensitivity}$ to define the cost of removing the filter, and the filter with the lowest ${Sensitivity}$ should be removed first to minimize the cost.
The ${Sensitivity}$ of each filter is calculated using Equation \ref{formula:taylor}.
\clr{I thought equation 4 is what the Tyler algorithm provided? is this a new metric we proposed? if this part is so closely related to section 3, we may just put it in section 3.}


We can rank the filters in ascending order by ${Sensitivity}$ to get the ranking of each filter and determine the removed order according to the ranking.
${Sensitivity}$ is calculated by gradient, \clr{so there is randomness in ${Sensitivity}$ as well as the gradient. there is not randomness in gradient computation, is this resulted from the SGD? (from the Adam and the SGD)}
This means that the filter ranking may be different in the result of two calculations using the same training data.
The randomness of ${Sensitivity}$ will affect the ranking of filters and the pruning plan.
We define $Instability$ to evaluate this situation and the equation is as follow:
\clr{We define \textit{Instability} as the variance of the filters' ranks from different computations, i.e.,}
\begin{equation}
     Instability(filter_j) = \frac{\sum_{i=1}^{n}(Rank_{i}(filter_j) - \overline{Rank(filter_j)})^2}{n}
\end{equation}
where $n$ is the calculation times of ranking, while $Rank_{i}(filter_j)$ is the index of the $filter_j$ in the $i$th ranking result, and $\overline{Rank(filter_j)}$ is the average index in all rankings.
The filter with high instability usually indicates that it is unimportant.



\subsection{Degeneration Exemplars and Evolution Exemplars}
\clr{add the figure from your slides into this section}
After pruning, the accuracy of the model for the test dataset is changed.
For test images, the prediction results between the original model and the pruning model may be changed.
Therefore, the following concepts are used in our work to describe those items.

\begin{flushleft}
\textbf{Degeneration Exemplars.} We use this term to represent the images that are correct in the original model and incorrect in the pruning model. 
After pruning, the recognition ability of the model on these images is degraded.
\end{flushleft}

\begin{flushleft}
\textbf{Evolution Exemplars.} We use this term to represent the images that are incorrect in the original model and correct in the pruning model. 
After pruning, the recognition ability of the model on these images is evolved.
\end{flushleft}



% Degeneration instances and  Evolution instances
% The system helps users select automatic pruning plans and generate a basic pruning process tree through visual analysis. Through the display of time-series statistics, users can quickly understand the state changes of the model and select a tree node as the start point for manual optimization. The system can help users to determine the number of filter deletions in the next step through an estimator. The visualization of each layer and the filter visualization can help the user to understand the pruning more deeply and refine the pruning scheme. After several manual pruning, users can get the desired compressed CNN model. We use comprehensive case studies on the CNNs with real-world sizes to validate the effectiveness of \sysname{}.




%After the user sets the auto-pruning parameters which can be determined through the information in the right views of the system, and the system can generate a basic tree through automatic pruning. Based on the information displayed in this basic tree, the user can select a node as the start point and make a pruning plan by using the estimator and model detail information. Finally, the user can get the target model through the iterative pruning.

% design:[goal, visual encoding]
%Model pruning is an iterative process, which requires multiple pruning and fine-tuning. (\clr{The first sentence conveys little information related to this view.}) To track the whole pruning process, we use the \textit{Tree} view (Fig. \ref{fig:teaser}-a) to display the information. In this process, there will be many intermediate models, and these models are dependent on each other, so using a tree to represent the iterative pruning can accurately express this process. The root node of the tree is the pre-trained model, and the others are pruned models. For a pruned model, the most concerned by the user about the model is the accuracy and compression rate. Therefore, We use a rectangle composed of three rectangles to represent the nodes in the tree, where the number in the left rectangle is the model id, the upper right rectangle represents the accuracy rate and the lower right rectangle represents the compression rate. The user can quickly understand the model overview and filter the model according to the goal through the display of these key information. In the tree, the child node is obtained by pruning the parent node, and the model needs to be fine-tuning after pruning. In the process of fine-tuning, whether the model meets the convergence conditions set by users is helpful for users to understand the stability and recovery ability of the model. In our design, we use lines of different colors to represent convergence results and the colors are black and red (\clr{I didn't see black lines? you mean blue and red?}). The black line indicates that the fine-tuning process after pruning from the parent node to the child node reaches the convergence condition which is set by the user, and the red line indicates the fine-tuning process achieves the maximum number of epoch without convergence. The user prunes the model by deleting the filters. To show the change of the number, we use the axis in the \textit{Tree} View to display the number of filters, and the axis only shows the numbers corresponding to the model in the tree. The toolbar is on the upper side of the \textit{Tree} View.



% interaction
%With the decrease of the filters, the over-parameterization of the model also decreases. When the filters reduced to a certain extent, the accuracy of the model begins to decrease. After many experiments, we find that the relationship between the accuracy and the number of filters tend to be a linear function in the later stage of pruning. Therefore, we design an estimator with a linear function to estimate the accuracy and compression between adjacent nodes. The estimator can be displayed or hidden by click the icon in the upper right corner of the \textit{Tree} view. The user can drag the estimator to any number of filters and the estimator performs linear interpolation according to the attributes of the two most adjacent nodes to get the estimated value. With this estimator, the user can determine the next pruning number according to the estimated value and some information in the right view. The user can switch the content of the right views by clicking the node in the tree.




% \clr{ The \textit{Tree} view provides an overview for the iterative model pruning process. The root and leaves of the tree are the original and pruned model respectively. Each branch of the tree (connecting the root to a leaf) chains a sequence of intermediate models from the iterative pruning process. For each node, we use two horizontal filled rectangles to denote the corresponding model's compression ratio and prediction accuracy. The vertical position of a node is decided by the number of filters in the corresponding model (see the left vertical axis). The edges connecting a pair of parent-child nodes represents the fine-tuning process, where we use black and red lines to indicate if the fine-tuning process converged or not after reaching the user-specified stop conditions (e.g., maximum number of epochs). Can you add interactions here? }

%\clr{ The \textit{Tree} view is also equipped with a pruning estimator, to help users balance the trade-off between model size and prediction accuracy. It estimates the number of filters in a model and the model's prediction accuracy, by linearly interpreting these values from a pair of most adjacent parent-child nodes from the tree. This rough linear estimation works well based on our experiments, and we expect more sophisticated interpretation algorithms to yield better results. The pruning estimator node is only visible when users pressing the icon (which?) on the top right corner of the tree view, and users can flexibly drag it vertically to dynamically generate the estimations.}


% In this task, the experts hope that our system can optimize the pruning strategy to help the model reduce the accuracy of category `buildings' less.
% In this case study, we show how to use {\sysname{}} to thoroughly analyze the model and optimize the pruning strategy.

